Effective Sample Size and Generalization Bounds for Temporal Networks

Learning from time series is fundamentally different from learning from i.i.d.\ data: temporal dependence can make long sequences effectively information-poor, yet standard evaluation protocols conflate sequence length with statistical information. We propose a dependence-aware evaluation methodology that controls for effective sample size $N_{\text{eff}}$ rather than raw length $N$, and provide end-to-end generalization guarantees for Temporal Convolutional Networks (TCNs) on $\beta$-mixing sequences. Our analysis combines a blocking/coupling reduction that extracts $B = \Theta(N/\log N)$ approximately independent anchors with an architecture-aware Rademacher bound for $\ell_{2,1}$-norm-controlled convolutional networks, yielding $O(\sqrt{D\log p / B})$ complexity scaling in depth $D$ and kernel size $p$. Empirically, we find that stronger temporal dependence can \emph{reduce} generalization gaps when comparisons control for $N_{\text{eff}}$ - a conclusion that reverses under standard fixed-$N$ evaluation, with observed rates of $N_{\text{eff}}^{-0.9}$ to $N_{\text{eff}}^{-1.2}$ substantially faster than the worst-case $O(N^{-1/2})$ mixing-based prediction. Our results suggest that dependence-aware evaluation should become standard practice in temporal deep learning benchmarks.

==> 6-discussion.tex <==
\section{Discussion} \label{sec:discussion}
Our results support a single overarching message: in temporal learning, \textbf{dependence changes the information budget}, and standard fixed-length evaluation can therefore lead to confounded and even reversed conclusions. Accordingly, we view the contributions in three layers: (i) a \textbf{fair-comparison protocol} that matches effective sample size $N_{\mathrm{eff}}$ across dependence strengths; (ii) an empirical finding that, under matched information, stronger dependence can \textbf{reduce} generalization gaps in our setting;
(iii) an architecture-aware theoretical baseline for dependent data that is valid but conservative.

\textbf{Fair comparison is the primary contribution.} For AR(1), matching effective information uses$N_{\mathrm{eff}} \approx N \cdot \frac{1-\rho}{1+\rho}.$ This makes explicit that holding $N$ fixed while varying $\rho$ changes the amount of usable information. In our grid (Table~\ref{tab:fair_comparison_lengths}), achieving the same $N_{\mathrm{eff}}$ requires up to a $\sim 6\times$ difference in raw length between $\rho=0.2$ and $\rho=0.8$, so fixed-$N$ comparisons can systematically favor weaker dependence simply because it provides more effective samples. This is exactly why the conclusions can reverse under the fair protocol (Section~\ref{subsec:standard_vs_fair}).

\textbf{Dependence can help once information is matched (in our setting).} Under fair comparison, we observe that stronger dependence can lead to smaller empirical gaps. At $N_{\mathrm{eff}}=2000$, $\rho=0.8$ yields a substantially smaller gap than $\rho=0.2$ (about a $76\%$ reduction; see Section~\ref{subsec:fair_results} and Figure~\ref{fig:fair_comparison}). This suggests that, for the AR(1) we study, TCN inductive bias can exploit temporal regularities rather than being uniformly harmed by dependence. Importantly, the fitted scaling exponents differ across $\rho$ (Figure~\ref{fig:fair_comparison}), indicating that the dependence-generalization relationship is nuanced and not captured by a single monotone trend.

\textbf{Role of the theory: conservative baseline, not a tight predictor.} The bound we develop is designed as a \textbf{valid worst-case reference} that cleanly exposes how architectural capacity (norm control, depth) and dependence (blocking/mixing) enter. Consistent with this goal, it is conservative in absolute magnitude in both synthetic and real-data settings (Figures~\ref{fig:fair_comparison} and~\ref{fig:physionet_gap_vs_N}). The empirical power-law behaviors (e.g., faster-than-$N^{-1/2}$ decay) should therefore be read as evidence of additional problem-dependent structure that the baseline does not model, rather than as a failure of correctness.

\textbf{Limitations.}
(i) The clean $N_{\mathrm{eff}}$ matching protocol relies on a known dependence-to-information relationship (here AR(1)), extending this to general processes requires robust estimators of effective information. (ii) Our main controlled findings are for TCNs; other architectures (e.g., attention) may behave differently. (iii) On real ECG signals we cannot manipulate dependence, so those experiments probe scaling and conservatism of the bound rather than dependence comparisons (Figures~\ref{fig:physionet_gap_vs_N}--\ref{fig:physionet_gap_vs_D}).On the theoretical side, (iv) our bounds require exponential $\beta$-mixing (Assumption~\ref{ass:exp_mixing}), which may not hold for all temporal processes.

